Theoretical Analysis of Bayesian Optimisation with Unknown Gaussian Process Hyper-Parameters

Bayesian optimisation has gained great popularity as a tool for optimising the parameters of machine learning algorithms and models. Somewhat ironically, setting up the hyper-parameters of Bayesian optimisation methods is notoriously hard. While reasonable practical solutions have been advanced, they can often fail to find the best optima. Surprisingly, there is little theoretical analysis of this crucial problem in the literature. To address this, we derive a cumulative regret bound for Bayesian optimisation with Gaussian processes and unknown kernel hyper-parameters in the stochastic setting. The bound, which applies to the expected improvement acquisition function and sub-Gaussian observation noise, provides us with guidelines on how to design hyper-parameter estimation methods. A simple simulation demonstrates the importance of following these guidelines.

==> proof_for_optimization.tex <==
\subsection{Theorems}
Let $C_2 := \prod_{i=1}^{d} \frac{\theta^U_i}{\theta^L_i}$.
Define $(R^L_T)^2 := C_2\|f\|^2_{\calH_{\vtheta^U}(\calX)} 
+ 2\log\left(\frac{t}{\sigma^2}\right)\gamma^{\vtheta^L}_t +  
\sqrt{8} \log\left(\frac{t}{\sigma^2}\right) \log^{1/2}(4k t^2 \pi^2/6\delta) 
\left(\sigma C_2 \|f\|_{\calH_{\vtheta^U}(\calX)} + \sqrt{\gamma^{\vtheta^L}_t}\right) + 
2 \log\left(\frac{t}{\sigma^2}\right) \sigma \log(2k t^2\pi^2/6\delta).$

\begin{theorem}
	Suppose $\vtheta^L \leq \vtheta_t \leq \vtheta^U$
	and $f \in \calH_{\vtheta^U}(\calX)$.
	If $\left(\nu_{t}^{\vtheta_{t}}\right)^2 = \vTheta \left( 2\gamma^{\vtheta_{t}}_T +  
		\sqrt{8} \log^{1/2}(4k T^2 \pi^2/6\delta) 
		\sqrt{\gamma^{\vtheta_{t}}_T}
		 + 2\sigma \log(2k T^2\pi^2/6\delta) \right)$.
	Then with probabily at least $1-\delta$,
	$R = \calO\left( R_{T}^{L} \sqrt{\gamma^{\vtheta^L}_T T}\right)$.
\end{theorem}
\begin{proof}
	First, let us assume that 
	$|\mu_t(\vx, \vtheta_{t}) - f(\vx)| \leq R_{t}^{\vtheta_{t}}\sigma_t(\vx; \vtheta_{t})$
	$\forall t \in \mathbb{N}, \vx \in \calX$. 
	By Proposition~\ref{prop:bound} and union bound, this hold with probability
	at least $\sum_{t=1}^{\infty}\frac{6\delta}{\pi^2 t^2} = \delta$.
	The regret at round $t$ is
	\begin{eqnarray}
		r_t &=& f^* - f(\vx_t) \nonumber \\
		&=& (f^* - \mu_{\vtheta_{t}}^*)- (f(\vx_t) - \mu_{\vtheta_{t}}^*) \nonumber  \\
		&\leq& I^{\vtheta_{t}}_t(\vx^*) + (\mu_{\vtheta_{t}}^* - \mu_{t}(\vx_t; \vtheta_t)) + 
			R_{t}^{\vtheta_{t}}\sigma_t(\vx_t; \vtheta_{t})
		\label{eqn:20}
	\end{eqnarray}
	By Lemma~\ref{lem:eikey}, we have that $I^{\vtheta_{t}}_t(\vx^*) \leq
	\frac{\tau(R_{t}^{\vtheta_{t}}/\nu_{t}^{\vtheta_{t}})}{\tau(-R_{t}^{\vtheta_{t}}/\nu_{t}^{\vtheta_{t}})}
	\alpha^\textrm{EI}_{\vtheta_{t}}(\vx^*|\data_t)$.
	By assumption $\left(\nu_{t}^{\vtheta_{t}}\right)^2 = \vTheta \left( 2\gamma^{\vtheta_{t}}_T +  
	\sqrt{8} \log^{1/2}(4k T^2 \pi^2/6\delta) 
	\sqrt{\gamma^{\vtheta_{t}}_T}
	+ 2\sigma \log(2k T^2\pi^2/6\delta) \right)$.
    Therefore, there exist $C$ such that
    $\left(\frac{\tau(R_{t}^{\vtheta_{t}}/\nu_{t}^{\vtheta_{t}})}
    	{\tau(-R_{t}^{\vtheta_{t}}/\nu_{t}^{\vtheta_{t}})}\right) \leq C$.
	By Lemma~\ref{lem:10}, we also have that 
	$(\mu_{\vtheta_{t}}^* - \mu_{t}(\vx_t; \vtheta_t)) 
	\leq \sqrt{\log\left(\frac{t+\sigma^2}{\sigma^2}\right)}  
	\nu_{t}^{\vtheta_{t}} \sigma_t(\vx_t; \vtheta_{t})$.

	Therefore, 
	\begin{eqnarray}
		\ref{eqn:20} &\leq& 
			C \alpha^\textrm{EI}_{\vtheta_{t}}(\vx^*|\data_t) + 
			\left(\sqrt{\log\left(\frac{t+\sigma^2}{\sigma^2}\right)} 
			\nu_{t}^{\vtheta_{t}} + R_{t}^{\vtheta_{t}}\right)
			\sigma_t(\vx_t; \vtheta_{t}) \nonumber  \\
		&\leq& 
			C \alpha^\textrm{EI}_{\vtheta_{t}}(\vx|\data_t)
			+ \left(\sqrt{\log\left(\frac{t+\sigma^2}{\sigma^2}\right)} 
			\nu_{t}^{\vtheta_{t}} + R_{t}^{\vtheta_{t}}\right)
			\sigma_t(\vx_t; \vtheta_{t}) \nonumber  \\
		&\leq& 
			C \left(I^{\vtheta_{t}}_t(\vx) + (R_{t}^{\vtheta_{t}} + 
			\nu_{t}^{\vtheta_{t}})\sigma_t(\vx; \vtheta_{t})\right)
			+ \left(\sqrt{\log\left(\frac{t+\sigma^2}{\sigma^2}\right)} 
			\nu_{t}^{\vtheta_{t}} + R_{t}^{\vtheta_{t}}\right)
			\sigma_t(\vx_t; \vtheta_{t}) \nonumber  \\
		&=& C I^{\vtheta_{t}}_t(\vx) 
			+ \left( (C+1) R_{t}^{\vtheta_{t}} + 
			\left(C+\sqrt{\log\left(\frac{t+\sigma^2}{\sigma^2}\right)} \right) 
			\nu_{t}^{\vtheta_{t}}\right)
			\sigma_t(\vx; \vtheta_{t}) \nonumber  \\
		&\leq& 
			C (\mu_t(\vx, \vtheta_{t}) + 
			R^{\vtheta_{t}}_t\sigma_t(\vx; \vtheta_{t}) - \mu_{\vtheta_{t}}^*)^+ 
			\nonumber \\
			&& + \left( (C+1) R_{t}^{\vtheta_{t}} + 
			\left(C+\sqrt{\log\left(\frac{t+\sigma^2}{\sigma^2}\right)} \right) 
			\nu_{t}^{\vtheta_{t}}\right)
			\sigma_t(\vx; \vtheta_{t}) \nonumber  \\
		&\leq& 
			\left( (2C+1) R_{t}^{\vtheta_{t}} + 
			\left(C+\sqrt{\log\left(\frac{t+\sigma^2}{\sigma^2}\right)} \right) 
			\nu_{t}^{\vtheta_{t}}\right)
			\sigma_t(\vx; \vtheta_{t}) \nonumber  \label{eqn:long1}
	\end{eqnarray}
	To simplify notation, let $t_0$ be such that
	$\log\left(\frac{t_0}{\sigma^2}\right) > 1$ and WLOG assume $C > 1$.
	Then
	\begin{eqnarray}
		\sum_{t=t_0}^{T}r_t^2 
		&\leq& \sum_{t=t_0}^{T} (2C+1)^2
			\left(R_{t}^{\vtheta_{t}} + 
			\sqrt{\log\left(\frac{t}{\sigma^2}\right)}\nu_{t}^{\vtheta_{t}} \right)^2
			\sigma_t^2(\vx; \vtheta_{t}) \nonumber \\
		&\leq& \sum_{t=t_0}^{T} (2C+1)^2
			\left((R_{t}^{\vtheta_{t}})^2 + 
			\log\left(\frac{t}{\sigma^2}\right) (\nu_{t}^{\vtheta_{t}})^2\right) 
			\sigma_t^2(\vx; \vtheta_{t}) \nonumber \\
		&\leq& \sum_{t=t_0}^{T} (2C+1)^2
			\left((R_{t}^{\vtheta_{t}})^2 
			+ \log\left(\frac{t}{\sigma^2}\right)(\nu_{t}^{\vtheta_{t}})^2\right) \sigma_t^2(\vx; \vtheta^{L}) 
			\label{eqn:11}
		% &\leq& 3C^2 ((R_{T}^{\vtheta})^2 + (\nu_{T}^{\vtheta})^2 + 1) \gamma^{\vtheta^L}_T.
	\end{eqnarray}
	By Lemma~\ref{lem:small}, we know that 
	$\rnorm{f}^2 \leq C_2 \|f\|^2_{\calH_{\vtheta^U}(\calX)}$.
	Also, by Lemma~\ref{lem:les}, $\gamma^{\vtheta_{t}}_t \leq \gamma^{\vtheta^L}_t$.
	Therefore, 
	$(R_{t}^{\vtheta_{t}})^2 \leq \left(R^L_T\right)^2.$
	Similarly, 
	$\log\left(\frac{t}{\sigma^2}\right)(\nu_{t}^{\vtheta_{t}})^2 
	= \calO \left( \left(R^L_T\right)^2 \right).$
	Then, 
	\begin{eqnarray*}
		\ref{eqn:11} 
		% &\leq& \sum_{t=1}^{T} (2C+1)^2
		% 	((R_{t}^{\vtheta_{t}})^2 
		% 	+ \log\left(\frac{t}{\sigma^2}\right)
		% 	(\nu_{t}^{\vtheta_{t}})^2) \sigma_t^2(\vx; \vtheta^{L}) \\
		&\leq& (2C+1)^2 \max_{t \in \{1, \cdots, T\}}
			\left[ (R_{t}^{\vtheta_{t}})^2 
			+ \log\left(\frac{t}{\sigma^2}\right)
			(\nu_{t}^{\vtheta_{t}})^2 \right] 
			\sum_{t=1}^{T} \sigma_t^2(\vx; \vtheta^{L}) \\
		&\leq&\calO \left( (R^L_T)^2 \gamma^{\vtheta^L}_t \right).
	\end{eqnarray*}
	% The last inequality holds by Lemma~\ref{lem:54} and the fact that 
	% $\max_{t \in \{1, \cdots, T\}}
	% \left[ (4(R_{t}^{\vtheta_{t}})^2 + (\nu_{t}^{\vtheta_{t}})^2 + 1) \right] 
	% = \calO\left( (R^L_T)^2 \right)$.
	Finally, by Cauchy-Schwarz inequality we have that 
	$R^2_T \leq T \sum_{t=1}^{T}r_t^2$ which concludes the proof.
\end{proof}
